Geodesic length and shifted weights in first-passage percolation

We study first-passage percolation through related optimization problems over paths of restricted length. The path length variable is in duality with a shift of the weights. This puts into a convex duality framework old observations about the convergence of the normalized Euclidean length of geodesics due to Hammersley and Welsh, Smythe and Wierman, and Kesten, and leads to new results about geodesic length and the regularity of the shape function as a function of the weight shift. For points far enough away from the origin, the ratio of the geodesic length and the $\ell^1$ distance to the endpoint is uniformly bounded away from one. The shape function is a strictly concave function of the weight shift. Atoms of the weight distribution generate singularities, that is, points of nondifferentiability, in this function. We generalize to all distributions, directions and dimensions an old singularity result of Steele and Zhang for the planar Bernoulli case. When the weight distribution has two or more atoms, a dense set of shifts produce singularities. The results come from a combination of the convex duality, the shape theorems of the different first-passage optimization problems, and modification arguments.

==> AsymOptMacros.tex <==
%%%%   In Ar-Fi-Ti 

%\RequirePackage{datetime} %comment out when arxiving or submitting

\usepackage{filemod}

\usepackage{amsmath,amssymb,amsthm,tikz,pgfplots} %,CJKutf8}
%\usepackage{showkeys}
%\usepackage[notref,notcite]{showkeys}
\usepackage[numbers,comma,square,sort&compress]{natbib}
\RequirePackage{color}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\definecolor{nicos-red}{rgb}{0.75,0.0,0.0}
\RequirePackage[colorlinks,urlcolor=my-blue,linkcolor=my-red,citecolor=my-green]{hyperref}
%\usepackage{enumerate}
\usepackage{enumitem}

\usetikzlibrary{arrows,patterns}


%how to label:  \begin{enumerate} [label=\rm(\roman{*}), ref=\rm(\roman{*})]
%alph

\usepackage{xargs}
\usepackage[colorinlistoftodos,prependcaption,textsize=footnotesize]{todonotes}
\newcommandx{\addmath}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommandx{\fixtext}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommandx{\anote}[2][1=]{\todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{#2}}

\usepackage{pdfcomment}

\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work 
\usepackage{accents} %for the interior of a set

%\usepackage{chngcntr}
%\counterwithin{equation}{chapter}
\numberwithin{figure}{section}

%\usepackage{parskip}   %% has the effect of putting space between par's and not indenting 

%\nofiles

%%%%%%%%
%%%%%  Let's specify these quantities in each paper file instead of in the common definitions file  
%%%%%%%%%
%\addtolength{\hoffset}{-.5in} 
%\addtolength{\textwidth}{1.6in}
%\addtolength{\oddsidemargin}{-0.3in}
%\addtolength{\evensidemargin}{-0.3in}
%\addtolength{\textheight}{0.8in}
%\addtolength{\topmargin}{-0.4in}
\addtolength\marginparwidth{-.4in}
%

%\addtolength{\footskip}{.3in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\evensidemargin}{0in}
%\setlength{\footskip}{0.2in}
%\setlength{\topmargin}{0.5in}
%\addtolength{\textheight}{.5in}


%\baselineskip=20pt  %% spread out text a little 

%NSF settings
%\setlength\hoffset{0pt}
%\setlength\voffset{0pt}
%\setlength\topmargin{0in}
%\setlength\evensidemargin{0in}
%\setlength\oddsidemargin{0in}
%\setlength\textwidth{6.5in}
%\setlength\headheight{0in}
%\setlength\headsep{.2in}
%\setlength\textheight{9in}
%\addtolength\textheight{-.2in}


\newtheorem{theorem}{\sc Theorem}[section]
\newtheorem{lemma}[theorem]{\sc Lemma}
\newtheorem{proposition}[theorem]{\sc Proposition}
\newtheorem{corollary}[theorem]{\sc Corollary}
\newtheorem{assumption}[theorem]{\sc Assumption}
\newtheorem{definition}[theorem]{\sc Definition}
%\newtheorem{remark}[theorem]{\sc Remark}
\numberwithin{equation}{section}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{problem}[theorem]{Problem}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}

\newcommand{\nn}{\nonumber}
\providecommand{\abs}[1]{\vert#1\vert}
\providecommand{\norm}[1]{\Vert#1\Vert}
\providecommand{\pp}[1]{\langle#1\rangle}
\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}

\newcommand{\sig}{{\scaleobj{0.8}{\boxempty}}} 
\newcommand{\sigg}{{\scaleobj{0.9}{\boxempty}}} 


%%generic definitions 
\def\cC{\mathcal{C}}  \def\cD{\mathcal{D}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cP{\mathcal{P}}
\def\cR{\mathcal{R}}
\def\cU{\mathcal{U}}
\def\cS{\mathcal{S}}
\def\cI{\mathcal{I}}
\def\cK{\mathcal{K}}
\def\cB{\mathcal{B}}
\def\cL{\mathcal{L}}
\def\cA{\mathcal{A}} \def\cV{\mathcal{V}}
\def\xhat{{\hat x}}
\def\uhat{{\hat u}}  \def\vhat{{\hat v}}
\def\wz{\eta}
\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\essinf{\mathop{\mathrm{ess\,inf}}}
\def\gr{\mathcal G}
\font \mymathbb = bbold10 at 11pt
\def\Hbar{\bar H}
\def\Phat{\widehat\P}
\def\Omhat{\widehat\Omega}
\def\kShat{\widehat\kS}
\def\That{\hat T}
\def\Bhat{\hat B}
\def\Vhat{\hat V}
\def\wzhat{\hat\wz}
\def\what{\hat\w}

\def\mbar{\wb m}   %% testing which bar looks best on m.  

%\newcommand{\one}{{{\rm 1\mkern-2.1mu}\!{\rm I}}}
\newcommand{\one}{\mbox{\mymathbb{1}}}


\def\kS{\mathfrak{S}}

\def\bB{{\mathbb B}}
\def\bE{\mathbb{E}}
\def\bN{\mathbb{N}}
\def\bP{\mathbb{P}}
\def\bQ{\mathbb{Q}}
\def\bR{\mathbb{R}}
\def\bZ{\mathbb{Z}}
\def\Zb{\mathbb{Z}}
\def\bI{\mathbb{I}}
\def\bV{{\mathbb V}}

\def\bS{\mathbb{S}}
 \def\Z{\bZ} \def\Q{\bQ} \def\R{\bR}\def\N{\bN}
  \def\evec{\mathbf{e}}  \def\uvec{\mathbf{u}}\def\vvec{\mathbf{v}}
    \def\kvec{\mathbf{k}}
 \def\zevec{\mathbf{0}}     

\def\ntil{\tilde{n}}
\def\xtil{\tilde{x}}
\def\xvec{\mathbf{x}}
\def\yvec{\mathbf{y}}
\def\zvec{\mathbf{z}}
\def\Yvec{\mathbf{Y}}  \def\Zvec{\mathbf{Z}} \def\thvec{\boldsymbol{\theta}}
\def\qbar{\bar{q}}
\def\Ybar{\bar{Y}}
\def\w{\omega}
\def\om{\omega}
\def\taubar{\bar{\tau}}
\def\omvec{\bar\omega}
\def\psibar{\overline\psi} 
\def\e{\varepsilon}
\def\ind{\mathbf{1}}
\def\ddd{\displaystyle} 

\def\mE{\mathbf{E}}   
\def\mH{\mathbf{H}}
\def\mP{\mathbf{P}}
\def\m1{\mathbf{1}}
\def\Ustat{\theta}
\def\Vstat{\beta}
\def \sqn{\sqrt{n}}

%%new def's 
 \def\Vvv{{\rm\mathbb{V}ar}}  \def\Cvv{{\rm\mathbb{C}ov}} 
 \def\hfun{h}
 \def\cJ{\mathcal{J}}  
 \def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline}
 \def\wc{\widecheck}
 \def\qvar{\sigma_0}
  \def\chfn{\lambda}  %%char function
 \def\bT{\mathbb{T}} 
 
%%notation specific to this material 
\def\E{\bE}
\def\P{\bP} %% environment measure 
\def\wlev{\omvec} %environment at a level 
\def\shift{\theta}  %spatial shift  
\def\refl{R}  %reflection of environment 
\def\nbhd{\cR}  %set of admissible steps 
\def\jump{v} %jump variable chosen from transition for couplings
\def\flux{H}   %macroscopic flux
\def\vva{v_0} \def\vvb{v_1}   %%%intersections at level j 
\def\north{S_{\mathcal N}}  \def\south{S_{\mathcal S}}  \def\east{S_{\mathcal E}}  
\def\west{S_{\mathcal W}}  
 
\def\OSP{(\Omega, \kS, \P)}
\def\backpi{\overleftarrow{\pi}} 
\def\backx{\overleftarrow{x}}
%\def\backx{\overset{\leftarrow}{x}}
\def\backX{\overleftarrow{X}}
%\def\backpi{\overset{\leftarrow}{\pi}}
\def\Zalt{Z^{\scriptscriptstyle\,\square}}
\def\Zalttil{\wt Z^{\scriptscriptstyle\,\square}}
\def\digamf{\Psi_0} %digamma function 
\def\trigamf{\Psi_1} %trigamma function 
\def\funct lp{L} %a function needed
\def\funct lpbar{\bar L} %a function needed

\def\note#1{{\color{red}(#1)}} 
\def\pfnote#1{{\color{red}{\bf((} #1 {\bf))}}}
\def\Nnote#1{{\color{nicos-red}{\bf((} #1 {\bf))}}}
\def\Fnote#1{{\color{orange}{\bf((} #1 {\bf))}}}

%Firas' notation
%\def\Dset{\mathbb D}
\def\Dset{\mathcal D}
\def\wDset{\Dset^{\,\wild}}
\def\zDset{\Dset^o}
\def\saDset{\Dset^{\text{\,{\rm{sa}}}}}
\def\Kop{{\mathbf s}}    %%% a function on cocycles 
\def\Aop{{\mathbf a}}    %%% another function on cocycles  ("Arjun")  
\def\zKop{\Kop^o}
\def\wKop{\Kop^{\wild}}
\def\range{\mathcal R}
\def\wrange{\mathcal R^{\wild}}
\def\zrange{\mathcal R^o}
\def\Paths{\Pi}
\def\zPaths{\Pi^o} 
\def\saPaths{\Pi^{\text{\rm{\,sa}}}} 
\def\saPathsS{\overline\Pi^{\text{\rm{\,sa}}}} 
\def\wPaths{\Paths^{\,\wild}} 

\def\cone{\mathcal C}
\def\Uset{\mathcal U}
\def\Vset{\mathcal V}

\def\G{\mathcal G}
\def\cA{\mathcal A}
\def\K{\mathcal K}
\def\L{\mathcal L}
\def\Yc{{\check Y}}
\def\Y{Y}
\def\necorner{{{}_\urcorner}}
\def\swcorner{{{}^\llcorner}}
\def\xexit{{m^{\swcorner}}}   %exit point from x-axis
\def\yexit{{n^{\swcorner}}}   %exit point from y-axis
%\def\dxexit{{m^{*,\swcorner}}  \def\dyexit{{n^{*,\swcorner}}}    %their duals
\def\xentrance{{m^{\necorner}}}   %entrance point to x-boundary
\def\yentrance{{n^{\necorner}}}   %entrance point  to y-boundary
\def\rect{{\mathfrak R}}
\def\V{{V}}
\def\Vw{V_0}   %%%% the part of the potential that depends only on \w 

 

\def\wild{\diamond}
\def\eee{\langle{\tt empty}\rangle} 
%\def\gpp{g_{\text{\rm{pp}}}}
\def\gpp{g}
\def\gppt{\psi}   %% shape function \gpp as a function of path length \tau
\def\wgppt{\psi^{\,\wild}} 
\def\zgppt{\psi^{o}} 
\def\Zpl{Z}
\def\Zpp{Z}
\def\Gpl{G}
\def\Gpp{G}
%\def\gs{{\bar g}_{\text{\rm{pp}}}}
\def\gs{\bar g}
\def\gpl{g_{\text{\rm{pl}}}}  

\def\wZpl{\Zpp^{\,\wild}}
\def\zZpp{\Zpp^{o}} 
\def\wZpp{\Zpp^{\,\wild}}
\def\wGpl{\Gpl^{\,\wild}}
\def\wGpp{\Gpp^{\,\wild}}
\def\wG{\Gpp^{\,\wild}}
\def\saG{\Gpp^{\text{\,\rm{sa}}}}
\def\wGpp{\Gpp^{\,\wild}}
\def\saGpp{\Gpp^{\text{\,\rm{sa}}}}
\def\GS{\overline\Gpp}
\def\saGS{{\GS}^{\text{\,\rm{sa}}}}
\def\wGS{{\GS}^{\,\wild}}
\def\saGSb#1{{\GS}^{\text{\,\rm{sa}},(#1)}}
\def\wgs{\gs^{\wild}}
\def\PathsS{\overline\Paths}
\def\wPathsS{\PathsS^{\,\wild}}
\def\TS{{\overline T}}
\def\TSb#1{\TS^{(#1)}}
\def\zGpp{\Gpp^o}
\def\zGS{\GS^o}
\def\sag{\gpp^{\text{\,\rm{sa}}}}
\def\sagb#1{\gpp^{\text{\,\rm{sa}},(#1)}}
\def\sagsb#1{\gs^{\text{\,\rm{sa}},(#1)}}
\def\sags{\gs^{\text{\,\rm{sa}}}}
\def\zgpp{\gpp^o} 
\def\zgppb#1{\gpp^{o,(#1)}}   %used for shifts 
\def\sagpp{\gpp^{\text{\rm{\,sa}}}}

\def\zgs{\gs^o} 
\def\bargpp{\gs}
\def\Lapp{\gpp}
%\def\barGpp{\wb\Gpp}   
\def\barGpp{\GS}
\def\tilGpp{\wt\Gpp}
\def\wgpp{\gpp^{\wild}}
\def\mus{\bar\mu}
\def\musb#1{\mus^{(#1)}}
\def\wgpl{\gpl^{\wild}}  
\def\Lapl{\gpl}
\def\gly{\mu}
\def\mgly{\gly^*}  %%%% maximum of shape function on bd of diamond
\def\dnfpp{H}  %dual norm of FPP 
\def\t{t}
\def\cut{c_0}
\def\cutt{c_1}
\def\Cut{C_0}
\def\Btil{\widetilde B}
\def\zero{\textcolor{red}0}
\def\Bpp{B_{\text{\rm{pp}}}}  
\def\Bpl{B_{\text{\rm{pl}}}} 
%\def\Lapl{\Lambda_{\text{\rm pl}}}
%\def\Lapp{\Lambda_{\text{\rm pp}}}
%\def\ri{{\mathrm{ri\,}}}
\def\f{{f}} %flux
%\def\zgppa{{\bar g}_{\text{\rm pp}}}
\def\zgppa{{\gamma}}
\def\amin{{\underline\alpha}}
\def\amax{{\overline\alpha}}
\def\nabmin{{\underline\nabla}}
\def\nabmax{{\overline\nabla}}
\def\h{{h}}
\def\hmin{{\underline h}}
\def\hmax{{\overline h}}
\def\smin{{\underline s}}
\def\smax{{\overline s}}
\def\ximin{{\underline\xi}}
\def\ximax{{\overline\xi}}
\def\Bmin{{\underline B}}
\def\Bmax{{\overline B}}
\def\Fmin{{\underline F}}
\def\Fmax{{\overline F}}
\def\zhat{{\hat z}}
\def\B{{B}}
\def\b{{b}}
\def\Bbar{{\bar\B}}
\def\cE{{\mathcal E}}

\def\G{{\mathbb G}}
\def\I{{I}}
\def\J{{J}}
\def\Yc{{\w}}
\def\W{{W}}
\def\S{{S}}
\def\A{{A}}
\def\M{{\mathcal M}}
\def\U{{U}}
\def\Ombig{{\widehat\Omega}}
\def\Pbig{{\widehat\P}}
\def\Ebig{{\widehat\E}}
\def\kSbig{{\widehat\kS}}
\def\www{{\bar\w}}
\def\PPP{{\overline\P}}
\def\EEE{{\overline\E}}
\def\Ommm{{\overline\Omega}}
\DeclareMathOperator{\ex}{ex}
%\DeclareMathOperator{\co}{co}
\def\O{{\mathcal O}}

\DeclareMathOperator{\hull}{\overline{\text{\rm{co}}}}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\bd}{bd}

\DeclareMathOperator{\sign}{sign} 
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\card}{card}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\Var}{Var}
  \DeclareMathOperator{\Cov}{Cov}  

\DeclareMathOperator{\proj}{Proj}
\DeclareMathOperator{\inter}{int}    % interior  
\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\intr}{int}    % interior  
\DeclareMathOperator{\rbd}{rbd} %rel boundary 
%\def\intU{\mathring\Uset} %interior of \Uset
%\newcommand\intr[1]{\accentset{\circ}{#1}}
\DeclareMathOperator{\aff}{aff}   %affine hull  
\DeclareMathOperator{\effdom}{dom}   %eff domain 
\DeclareMathOperator{\id}{id}

%% Arjun
% commenting command
%\newcommand{\arjun}[1]{\textcolor{blue}{arjun: #1}}

\newcommand{\biinfinite}{bi-infinite}

%\def\Zb{\mathbf{Z}}
\newcommand{\Eqref}[1]{\eqref{#1}}
\newcommand{\Figref}[1]{Fig.~\ref{#1}}
\newcommand{\Tabref}[1]{Table.~\ref{#1}}
\newcommand{\Secref}[1]{Section~\ref{#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{#1}}
\newcommand{\Corref}[1]{Corollary~\ref{#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{#1}}
\newcommand{\Propref}[1]{Prop.~\ref{#1}}
\newcommand{\Defref}[1]{Definition~\ref{#1}}
\newcommand{\Remref}[1]{Remark~\ref{#1}}
\newcommand{\Claimref}[1]{Claim~\ref{#1}}
\newcommand{\Itemref}[1]{Item~\ref{#1}}

% refresh emph command to be bold
\renewcommand{\emph}[1]{\textbf{#1}}

\newcommand{\AND}{\textrm{ and }} 
\newcommand{\OR}{\textrm{ or }}
\newcommand{\Prob}{\mathbb{P}} %probability 

\newcommand{\FPP}{first-passage percolation}
\newcommand{\FPT}{first-passage time}
% Other commads
\def\grad{\nabla}
\newcommand{\sgn}[1]{\text{sgn}(#1)}

%\def\int{\text{int}}
\def\H{\mathcal{H}}

\def\hatmu{\hat{\mu}}

\def\T{T}   % passage time
\def\Tb#1{T^{(#1)}}   % passage time
\newcommand{\Norm}[2]{\left|{#1}\right|_{#2}} %norm
\def\dualT{T^*}
\def\dualmu{\rho}

\def\lev{\sigma}  \def\rev{\tau}   %% left and right e-vectors  
\def\rectan{\Lambda}  %% rectangle 
\def\amatri{A}   %matrix for Perron-Frob  
\def\bmatri{A} 

\def\ellc{\delta}  %%% ellipticity constant 

 
 % the lower and upper bound on the "gap" interval:  "lambda inf" and "lambda sup".  Micro counterparts with \ell 
\def\lain{\underline\lambda} 
\def\lasu{\overline\lambda} 
\def\elin{\underline\ell} 
\def\elsu{\overline\ell} 

\def\aaV#1{V^{(#1)}}
\def\aaGpp#1{G^{(#1)}}                          %%%  weights shifted by #1
%\def\aagpp#1{g^{(#1)}_{\text{\rm{pp}}}} 
\def\aagpp#1{\gpp^{(#1)}} 
\def\aasag#1{\gpp^{\text{\rm{sa}},(#1)}} 
%\def\aaell#1{\fppell^{(#1)}}

\def\aalain#1{\lain^{(#1)}} 
\def\aalasu#1{\lasu^{\tspb(#1)}} 
\def\aaelin#1{\elin^{(#1)}}
\def\aaelsu#1{\elsu^{(#1)}}

\def\parng#1#2{#1\hspace{0.6pt}{\boldsymbol:}\hspace{0.3pt}#2}  %path range 


\def\zUset{\Uset^o}

\def\zgpl{g^o_{\text{\rm{pl}}}} 

\DeclareMathOperator{\conv}{co}   %convex hull  

\def\Ew{m_0} %mean of edge weight
\def\eit{r_0} %essinf of edge weight
\def\est{M_0} %esssup of edge weight
\def\eet{\e_0}  %the amount by which we can go below -\eit  
\def\bmin{b_0} %minimal shift with time constant > -\infty
\def\bmins{\bar b_0} %minimal shift with time constant > -\infty
\def\Sl{\cS} %slab

\def\Ca{A}  %constant for \bar B blocks 
\def\Cl{L}  %another constant 


\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkblue}{rgb}{0.0,0.0,0.3}
\definecolor{nicosred}{rgb}{0.65,0.1,0.1}
\definecolor{light-gray}{gray}{0.7}
\allowdisplaybreaks[1]


% Some macros for differentiability
\def\Bxi{B^{\xi}}
\def\Btheta{B^{\theta}}
\def\Bplus{B_+}
\def\Bminus{B_-}
\def\Bpm{B_\pm}

\def\xiplus{\xi_+}
\def\ximinus{\xi_-}
\def\xipm{\xi_\pm}

\def\Gplus{G_+}
\def\Gminus{G_-}
\def\Gpm{G_\pm}
\def\Gxi{G^{\xi}}
\def\Gtheta{G_{\theta}} % could be G_{\theta}^{\xi}

\def\Gstar{G^*}
\def\pistar{\pi^*}
\def\wstar{\w^*}
\def\barpi{\overline{\pi}}

\def\tautheta{\tau_{\theta}}
\def\taupm{\tau_{\pm}}

\def\deltaomega{\Delta\omega}

\newcommand{\deltaGpm}[2]{(G_-(#1) - G_-(#2)) - (G_+(#1) - G_+(#2))}
\newcommand{\DeltaGpm}{\Delta_\pm G}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\argmax}{argmax}

\newcommand{\arjunopt}[1]{\opt{notes}{\textcolor{OliveGreen}{arjun: #1}}}

% argmax
\def\argmax{\operatorname{argmax}}

\newcommand{\almostsurely}{\textrm{a.s}}

%%FPP notation 
\def\lell{\ell}
\def\tpath{T}   %passage time of a path 
\def\path{x_\bbullet}   %generic path
\def\sspath{x_\brbullet}   %generic path in subscript
\def\fppb{\gly}  %time constant as function of shift of weights 
%\def\fppc{\bar\fppb} 
\def\fppc{\overline\fppb}
\def\fppbs{\overline\phi}  %time constant as function of shift of weights 
\def\qedex{\hfill$\triangle$}    % at the end of remarks  and examples 
\def\ccm{m}  %cocycle mean vector 


\newcommand{\lzb}{\llbracket}   %left Z bracket  
\newcommand{\rzb}{\rrbracket}   %right Z bracket 

\newcommand\abullet{{\scaleobj{0.6}{\bullet}}}  %%%% smaller bullet to use inside functions 
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.5}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-0.5pt}{\scaleobj{0.4}{\bullet}}}} %%  for subscript paths x_\brbullet   need negative raise 
\newcommand\cbullet{{\raisebox{1pt}{\scaleobj{0.6}{\bullet}}}}

\newcommand\dbullet{{\scaleobj{0.7}{\bullet}}}   % same as \bbullet but without shift up

\newcommand\bcdot{{\scaleobj{1.8}{\cdot}}}
\newcommand\acdot{{\raisebox{-1pt}{\scaleobj{1.4}{\cdot}}}}  %%dot inside function 

\def\timonote#1{{\color{blue}{\bf(}#1 [Timo]{\bf)}}}

\def\tsp{\hspace{0.55pt}}  %this is sometimes a good spacing in formulas when \, is too large 
\def\tspa{\hspace{0.7pt}}  
\def\tspb{\hspace{0.9pt}}
\def\tspc{\hspace{1.1pt}}



\def\parQ{Q}  %a parameter coming along for the ride 
\def\vaa{v_1}
\def\vbb{w_1} %%% vertices 

\def\dtnr{k_0}  % fluffy nr of detours 
\def\exnr{\sigma}  % fluffy nr of excursions 
\def\param{s}   %a parameter for the vBK argument 



